A Backtracking-Based Algorithm for Computing Hypertree-Decompositions

Hypertree decompositions of hypergraphs are a generalization of tree decompositions of graphs. The corresponding hypertree-width is a measure for the cyclicity and therefore tractability of the encoded computation problem. Many NP-hard decision and computation problems are known to be tractable on instances whose structure corresponds to hypergraphs of bounded hypertree-width. Intuitively, the smaller the hypertree-width, the faster the computation problem can be solved. In this paper, we present the new backtracking-based algorithm det-k-decomp for computing hypertree decompositions of small width. Our benchmark evaluations have shown that det-k-decomp significantly outperforms opt-k-decomp, the only exact hypertree decomposition algorithm so far. Even compared to the best heuristic algorithm, we obtained competitive results as long as the hypergraphs are not too large.

==> graphics/depgraph.tex <==

\begin{figure}[t]
\begin{center}
 
\input{graphics/depgraph.pstex_t}

\caption{Dependency graph between procedures called by $k$-decomp}
\label{fig:depgraph}
\end{center}
\end{figure}



==> graphics/detkdecomp.tex <==


\begin{algorithm}
%\begin{algorithmic}
%\STATE
\begin{tabbing}
\hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.2cm} \= \hspace*{0.2cm} \= \kill

{\tiny \phantom{0}1} \> $\mathit{FailSeps} := \emptyset$; \\
{\tiny \phantom{0}2} \> $\mathit{SuccSeps} := \emptyset$; \\
{\tiny \phantom{0}3} \> $\mathit{HTree} := \mathit{decompCov}(\mathit{edges}(\mathit{HGraph}), \emptyset)$; \\
{\tiny \phantom{0}4} \> {\bf if} $\mathit{HTree} \not= \mathit{NULL}$ {\bf then} \\
{\tiny \phantom{0}5} \>\> $\mathit{HTree} := \mathit{expand}(\mathit{HTree})$; \\
{\tiny \phantom{0}6} \> {\bf endif} \\
{\tiny \phantom{0}7} \> {\bf return} $\mathit{HTree}$;

\end{tabbing}
%\end{algorithmic}
\caption{$\mathit{det}$-$k$-$\mathit{decomp}(\mathit{HGraph})$}
\label{alg:det-k-decomp}
\end{algorithm}



\begin{algorithm}
%\begin{algorithmic}
%\STATE
\begin{tabbing}
\hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.2cm} \= \hspace*{0.2cm} \= \kill

{\tiny \phantom{0}1} \> {\bf if} $|\mathit{Edges}| \leq k$ {\bf then} \\
{\tiny \phantom{0}2} \>\> $\mathit{HTree} := \mathit{getHTNode}(\mathit{Edges}, \bigcup \mathit{Edges}, \emptyset)$; \\
{\tiny \phantom{0}3} \>\> {\bf return} {\it HTree}; \\
{\tiny \phantom{0}4} \> {\bf endif} \\
{\tiny \phantom{0}5} \> $\mathit{BoundEdges} := \{e \in \mathit{edges}(\mathit{HGraph}) \;|\; e \cap \mathit{Conn} \not= \emptyset\}$; \\
{\tiny \phantom{0}6} \> {\bf for each} $\mathit{CovSep} \in \mathit{cover}(\mathit{Conn}, \mathit{BoundEdges})$ {\bf do} \\
{\tiny \phantom{0}7} \>\> $\mathit{HTree} := \mathit{decompAdd}(\mathit{Edges}, \mathit{Conn}, \mathit{CovSep})$; \\
{\tiny \phantom{0}8} \>\> {\bf if} $\mathit{HTree} \not= \mathit{NULL}$ {\bf then} \\
{\tiny \phantom{0}9} \>\>\> {\bf return} {\it HTree}; \\
{\tiny 10} \>\> {\bf endif} \\
{\tiny 11} \> {\bf endfor} \\
{\tiny 12} \> {\bf return} \it{NULL};

\end{tabbing}
%\end{algorithmic}
\caption{$\mathit{decompCov}(\mathit{Edges}, \mathit{Conn})$}
\label{alg:decompCov}
\end{algorithm}



\begin{algorithm}
%\begin{algorithmic}
%\STATE
\begin{tabbing}
\hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \kill

{\tiny \phantom{0}1} \> $\mathit{InCovSep} := \mathit{CovSep} \cap \mathit{Edges}$; \\
{\tiny \phantom{0}2} \> {\bf if} $\mathit{InCovSep} \not= \emptyset$ {\bf or} $k - |\mathit{CovSep}| > 0$ {\bf then} \\
{\tiny \phantom{0}3} \>\> {\bf if} $\mathit{InCovSep} = \emptyset$ {\bf then} $\mathit{AddSize} := 1$ {\bf else} $\mathit{AddSize} := 0$ {\bf endif}; \\
{\tiny \phantom{0}4} \>\> {\bf for each} $\mathit{AddSep} \subseteq \mathit{Edges}$ {\bf s.t.}\ $|\mathit{AddSep}| = \mathit{AddSize}$ {\bf do} \\
{\tiny \phantom{0}5} \>\>\> $\mathit{Separator} := \mathit{CovSep} \cup \mathit{AddSep}$; \\
{\tiny \phantom{0}6} \>\>\> $\mathit{Components} := \mathit{separate}(\mathit{Edges}, \mathit{Separator})$; \\
{\tiny \phantom{0}7} \>\>\> {\bf if} $\,\forall \mathit{Comp} \in \mathit{Components} .\,\langle\mathit{Separator},\mathit{Comp}\rangle \notin \mathit{FailSeps}$ {\bf then} \\
{\tiny \phantom{0}8} \>\>\>\> $\mathit{Subtrees} := \mathit{decompSub}(\mathit{Components}, \mathit{Separator})$; \\
{\tiny \phantom{0}9} \>\>\>\> {\bf if} $\mathit{Subtrees} \not= \emptyset$ {\bf then} \\
{\tiny 10} \>\>\>\>\> $\mathit{Chi} := \mathit{Conn} \cup \,\bigcup (\mathit{InCovSep} \cup \mathit{AddSep})$; \\
{\tiny 11} \>\>\>\>\> $\mathit{HTree} := \mathit{getHTNode}(\mathit{Separator}, \mathit{Chi}, \mathit{Subtrees})$; \\
{\tiny 12} \>\>\>\>\> {\bf return} \it{HTree}; \\
{\tiny 13} \>\>\>\> {\bf endif} \\
{\tiny 14} \>\>\> {\bf endif} \\
{\tiny 15} \>\> {\bf endfor} \\
{\tiny 16} \> {\bf endif} \\
{\tiny 17} \> {\bf return} {\it NULL};

\end{tabbing}
%\end{algorithmic}
\caption{$\mathit{decompAdd}(\mathit{Edges}, \mathit{Conn}, \mathit{CovSep})$}
\label{alg:decompAdd}
\end{algorithm}



\begin{algorithm}
%\begin{algorithmic}
%\STATE
\begin{tabbing}
\hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \kill

{\tiny \phantom{0}1} \> $\mathit{Subtrees} := \emptyset$; \\
{\tiny \phantom{0}2} \> {\bf for each} $\mathit{Comp} \in \mathit{Components}$ {\bf do} \\
{\tiny \phantom{0}3} \>\> $\mathit{ChildConn} := \bigcup\mathit{Comp} \cap \bigcup\mathit{Separator}$; \\
{\tiny \phantom{0}4} \>\> {\bf if} $\langle\mathit{Separator},\mathit{Comp}\rangle \in \mathit{SuccSeps}$ {\bf then} \\
{\tiny \phantom{0}5} \>\>\> $\mathit{HTree} := \mathit{getHTNode}(\mathit{Comp}, \mathit{ChildConn}, \emptyset)$; \\
{\tiny \phantom{0}6} \>\> {\bf else} \\
{\tiny \phantom{0}7} \>\>\> $\mathit{HTree} := \mathit{decompCov(Comp, ChildConn)}$; \\
{\tiny \phantom{0}8} \>\>\> {\bf if} $\mathit{HTree} = \mathit{NULL}$ {\bf then} \\
{\tiny \phantom{0}9} \>\>\>\> $\mathit{FailSeps} := \mathit{FailSeps} \cup \{\langle\mathit{Separator}, \mathit{Comp}\rangle\}$; \\
{\tiny 10} \>\>\>\> {\bf return} $\emptyset$; \\
{\tiny 11} \>\>\> {\bf else} \\
{\tiny 12} \>\>\>\> $\mathit{SuccSeps} := \mathit{SuccSeps} \cup \{\langle\mathit{Separator}, \mathit{Comp}\rangle\}$; \\
{\tiny 13} \>\>\> {\bf endif} \\
{\tiny 14} \>\> {\bf endif} \\
{\tiny 15} \>\> $\mathit{Subtrees} := \mathit{Subtrees} \cup \{\mathit{HTree}\}$; \\
{\tiny 16} \> {\bf endfor} \\
{\tiny 17} \> {\bf return} {\it Subtrees};

\end{tabbing}
%\end{algorithmic}
\caption{$\mathit{decompSub}(\mathit{Components}, \mathit{Separator})$}
\label{alg:decompSub}
\end{algorithm}



==> graphics/ex_callseq.tex <==

\begin{figure}[t]
\begin{center}

\input{graphics/ex_callseq.pstex_t}
\hspace*{6cm}
\input{graphics/ex_hyptree2.pstex_t}

\caption{A procedure call sequence and the corresponding hypertree decomposition}
\label{fig:ex_callseq}
\end{center}
\end{figure}



==> graphics/ex_cover.tex <==

\begin{figure}[t]
\begin{center}
 
\vspace*{2ex}
\input{graphics/ex_cover.pstex_t}

\caption{Covering $\mathit{Conn}=\{a,b,e\}$ by $\mathit{BoundEdges}=\{A,B,D,F,G,H\}$}
\label{fig:ex_cover}
\end{center}
\end{figure}



==> graphics/ex_hgraph.tex <==

\begin{figure}[t]
\begin{center}
 
\input{graphics/ex_hgraph.pstex_t}
\hspace*{0.8cm}
\input{graphics/ex_hyptree.pstex_t}

\caption{Example of a hypergraph and its hypertree decomposition of width~$2$}
\label{fig:ex_hgraph}
\end{center}
\end{figure}



==> graphics/kdecomp.tex <==


\begin{algorithm}
%\begin{algorithmic}
%\STATE
\begin{tabbing}
\hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.2cm} \= \hspace*{0.2cm} \= \kill

{\tiny \phantom{0}1} \> $\mathit{HTree}$ := $k$-$\mathit{decomposable}(\mathit{edges}(\mathit{HGraph}), \emptyset)$; \\
{\tiny \phantom{0}2} \> {\bf return} $\mathit{HTree}$;

\end{tabbing}
%\end{algorithmic}
\caption{$k$-$\mathit{decomp}(\mathit{HGraph})$}
\label{alg:k-decomp}
\end{algorithm}



\begin{algorithm}
%\begin{algorithmic}
%\STATE
\begin{tabbing}
\hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.4cm} \= \hspace*{0.2cm} \= \hspace*{0.2cm} \= \kill

{\tiny \phantom{0}1} \> {\bf guess} $\mathit{Separator} \subseteq \mathit{edges}(\mathit{HGraph})$ {\bf such that} $|\mathit{Separator}| \leq k$; \\
{\tiny \phantom{0}2} \> {\bf check} that the following two conditions hold: \\
{\tiny \phantom{0}3} \>\> $\bigcup \mathit{Edges} \cap \bigcup \mathit{OldSep} \subseteq \bigcup \mathit{Separator}$; \\
{\tiny \phantom{0}4} \>\> $\mathit{Separator} \cap \mathit{Edges} \not= \emptyset$; \\
{\tiny \phantom{0}5} \> {\bf if} one of these checks fails {\bf then return} $\mathit{NULL}$; \\
{\tiny \phantom{0}6} \> $\mathit{Components} := \mathit{separate}(\mathit{Edges}, \mathit{Separator})$; \\
{\tiny \phantom{0}7} \> $\mathit{Subtrees} := \emptyset$; \\
{\tiny \phantom{0}8} \> {\bf for each} $\mathit{Comp} \in \mathit{Components}$ {\bf do} \\
{\tiny \phantom{0}9} \>\> $\mathit{HTree} := k$-$\mathit{decomposable(Comp, Separator)}$; \\
{\tiny 10} \>\> {\bf if} $\mathit{HTree} = \mathit{NULL}$ {\bf then} \\
{\tiny 11} \>\>\> {\bf return} $\mathit{NULL}$; \\
{\tiny 12} \>\> {\bf else} \\
{\tiny 13} \>\>\> $\mathit{Subtrees} := \mathit{Subtrees} \cup \{\mathit{HTree}\}$; \\
{\tiny 14} \>\> {\bf endif} \\
{\tiny 15} \> {\bf endfor} \\
{\tiny 16} \> $\mathit{Chi} := (\bigcup \mathit{Edges} \cap \bigcup \mathit{OldSep}) \cup \,\bigcup (\mathit{Separator} \cap \mathit{Edges})$; \\
{\tiny 17} \> $\mathit{HTree} := \mathit{getHTNode}(\mathit{Separator}, \mathit{Chi}, \mathit{Subtrees})$; \\
{\tiny 18} \> {\bf return} {\it HTree};

\end{tabbing}
%\end{algorithmic}
\caption{$k$-$\mathit{decomposable}(\mathit{Edges}, \mathit{OldSep})$}
\label{alg:k-decomposable}
\end{algorithm}




==> graphics/memuse.tex <==

\begin{figure}[t]
\setlength{\unitlength}{1cm}

\begin{center}
\epsfig{file=graphics/s298-optkdec.eps, scale=0.58}
\hspace*{0.5cm}
\epsfig{file=graphics/s298-kdec.eps, scale=0.58}
\end{center}


\begin{center}
\vspace*{-2ex}
\begin{picture}(15.4,0.3)
\put(0,0){\makebox(5.85,0.4){(a) opt-$k$-decomp}}
\put(6.45,0){\makebox(5.85,0.4){(b) det-$k$-decomp}}
\end{picture}
\end{center}

\vspace*{-2ex}
\caption{CPU and memory usage when decomposing s298 of the ISCAS89 benchmarks}
\label{fig:memuse}
\end{figure}



==> graphics/strongnf.tex <==

\begin{figure}[t]
\begin{center}
 
\input{graphics/strongnf.pstex_t}

\caption{Transformation steps to strong normal form}
\label{fig:strongnf}
\end{center}
\end{figure}



==> graphics/tab_dc.tex <==

\setlength\extrarulesep{0.5ex}
\renewcommand{\multirowsetup}{\centering}

%\begin{table}
%\begin{sidewaystable}
%\begin{center}

\begin{tabular}{|l|c||c|c||c|c||c|c|}
\hline
\multirow{2}{6cm}{\vfill{\bf Instance} {\it (Atoms / Variables)}\vfill} & \multirow{2}{1.2cm}{\vfill{\bf Min}\vfill} & \multicolumn{2}{c||}{\bf opt-$k$-decomp} &  \multicolumn{2}{c||}{\bf BE} & \multicolumn{2}{c|}{\bf det-$k$-decomp} \\
\cline{3-8}
&& \hspace*{0.5ex}{\it Width}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Time}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Width}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Time}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Width}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Time}\hspace*{0.5ex} \\
\hline\hline

{\bf adder\_15} (76 / 106) & {\bf 2} & {\bf 2} & 5 & {\bf 2} & 0 & {\bf 2} & 0 \\
\hline
{\bf adder\_25} (126 / 176) & {\bf 2} & {\bf 2} & 40 & {\bf 2} & 0 & {\bf 2} & 0 \\
\hline
{\bf adder\_50} (251 / 351) & {\bf 2} & --- & --- & {\bf 2} & 0 & {\bf 2} & 0 \\
\hline
{\bf adder\_75} (376 / 526) & {\bf 2} & --- & --- & {\bf 2} & 0 & {\bf 2} & 0 \\
\hline
{\bf adder\_99} (496 / 694) & {\bf 2} & --- & --- & {\bf 2} & 1 & {\bf 2} & 0 \\
\hline
{\bf bridge\_15} (137 / 137) & {\bf 2} & {\bf 2} & 19 & {\bf 3} & 0 & {\bf 2} & 0 \\
\hline
{\bf bridge\_25} (227 / 227) & {\bf 2} & {\bf 2} & 138 & {\bf 3} & 0 & {\bf 2} & 0 \\
\hline
{\bf bridge\_50} (452 / 452) & {\bf 2} & {\bf 2} & 2211 & {\bf 3} & 1 & {\bf 2} & 0 \\
\hline
{\bf bridge\_75} (677 / 677) & {\bf 2} & --- & --- & {\bf 3} & 1 & {\bf 2} & 0 \\
\hline
{\bf bridge\_99} (893 / 893) & {\bf 2} & --- & --- & {\bf 3} & 2 & {\bf 2} & 1 \\
\hline
{\bf NewSystem1} (84 / 142) & {\bf 3} & --- & --- & {\bf 3} & 0 & {\bf 3} & 0 \\
\hline
{\bf NewSystem2} (200 / 345) & {\bf 3} & --- & --- & {\bf 4} & 0 & {\bf 3} & 0 \\
\hline
{\bf NewSystem3} (278 / 474) & --- & --- & --- & {\bf 5} & 1 & {\bf 4} & 0 \\ 
\hline
{\bf NewSystem4} (418 / 718) & --- & --- & --- & {\bf 5} & 2 & {\bf 4} & 0 \\ \hline
{\bf atv\_partial\_system} (88 / 125) & {\bf 3} & --- & --- & {\bf 3} & 0 & {\bf 3} & 0 \\
\hline

\end{tabular}
%\end{center}
%\caption{DaimlerChrysler benchmarks}
%\label{tab:dc}
%\end{sidewaystable}
%\end{table}

\setlength\extrarulesep{0pt}


==> graphics/tab_grid2d.tex <==

\setlength\extrarulesep{0.5ex}
\renewcommand{\multirowsetup}{\centering}

%\begin{table}
%\begin{sidewaystable}
%\begin{center}

\begin{tabular}{|l|c||c|c||c|c||c|c|}
\hline
\multirow{2}{6cm}{\vfill{\bf Instance} {\it (Atoms / Variables)}\vfill} & \multirow{2}{1.2cm}{\vfill{\bf Min}\vfill} & \multicolumn{2}{c||}{\bf opt-$k$-decomp} &  \multicolumn{2}{c||}{\bf BE} & \multicolumn{2}{c|}{\bf det-$k$-decomp} \\
\cline{3-8}
&& \hspace*{0.5ex}{\it Width}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Time}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Width}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Time}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Width}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Time}\hspace*{0.5ex} \\
\hline\hline

{\bf grid2d\_10} (50 / 50) & {\bf 4} & --- & --- & {\bf 5} & 0 & {\bf 4} & 0 \\
\hline
{\bf grid2d\_15} (112 / 113) & {\bf 6} & --- & --- & {\bf 8} & 0 & {\bf 6} & 3 \\
\hline
{\bf grid2d\_20} (200 / 200) & {\bf 7} & --- & --- & {\bf 12} & 0 & {\bf 7} & 3140 \\
\hline
{\bf grid2d\_25} (312 / 313) & {\bf 9} & --- & --- & {\bf 15} & 3 & {\bf 10} & 2000 \\
\hline
{\bf grid2d\_30} (450 / 450) & {\bf 11} & --- & --- & {\bf 19} & 7 & {\bf 13} & 1566 \\
\hline
{\bf grid2d\_35} (612 / 613) & {\bf 12} & --- & --- & {\bf 23} & 15 & {\bf 15} & 1905 \\
\hline
{\bf grid2d\_40} (800 / 800) & {\bf 14} & --- & --- & {\bf 26} & 28 & {\bf 17} & 2530 \\
\hline
{\bf grid2d\_45} (1012 / 1013) & {\bf 16} & --- & --- & {\bf 31} & 51 & {\bf 21} & 2606 \\
\hline
{\bf grid2d\_50} (1250 / 1250) & {\bf 17} & --- & --- & {\bf 33} & 86 & {\bf 24} & 2786 \\
\hline
{\bf grid2d\_60} (1800 / 1800) & {\bf 21} & --- & --- & {\bf 41} & 204 & {\bf 31} & 2984 \\
\hline
{\bf grid2d\_70} (2450 / 2450) & {\bf 24} & --- & --- & {\bf 48} & 474 & {\bf 42} & 2161 \\
\hline
{\bf grid2d\_75} (2812 / 2813) & {\bf 26} & --- & --- & {\bf 48} & 631 & {\bf 45} & 2881 \\
\hline

\end{tabular}
%\end{center}
%\caption{Grid2D benchmarks}
%\label{tab:grid2d}
%\end{sidewaystable}
%\end{table}

\setlength\extrarulesep{0pt}


==> graphics/tab_iscas89.tex <==

\setlength\extrarulesep{0.5ex}
\renewcommand{\multirowsetup}{\centering}

%\begin{table}
%\begin{sidewaystable}
%\begin{center}

\begin{tabular}{|l|c||c|c||c|c||c|c|}
\hline
\multirow{2}{6cm}{\vfill{\bf Instance} {\it (Atoms / Variables)}\vfill} & \multirow{2}{1.2cm}{\vfill{\bf Min}\vfill} & \multicolumn{2}{c||}{\bf opt-$k$-decomp} & \multicolumn{2}{c||}{\bf BE} & \multicolumn{2}{c|}{\bf det-$k$-decomp} \\
\cline{3-8}
&& \hspace*{0.5ex}{\it Width}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Time}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Width}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Time}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Width}\hspace*{0.5ex} & \hspace*{0.5ex}{\it Time}\hspace*{0.5ex} \\
\hline\hline

{\bf s27} (13 / 17) & {\bf 2} & {\bf 2} & 0 & {\bf 2} & 0 & {\bf 2} & 0 \\
\hline
{\bf s208} (104 / 115) & {\bf $\geq$ 3} & --- & --- & {\bf 7} & 0 & {\bf 6} & 0 \\
\hline
{\bf s298} (133 / 139) & {\bf $\geq$ 3} & --- & --- & {\bf 5} & 0 & {\bf 4} & 462 \\
\hline
{\bf s344} (175 / 184) & {\bf $\geq$ 3} & --- & --- & {\bf 7} & 0 & {\bf 5} & 730 \\
\hline
{\bf s349} (176 / 185) & {\bf $\geq$ 3} & --- & --- & {\bf 7} & 0 & {\bf 5} & 4 \\
\hline
{\bf s382} (179 / 182) & {\bf $\geq$ 3} & --- & --- & {\bf 5} & 0 & {\bf 5} & 722 \\
\hline
{\bf s386} (165 / 172) & --- & --- & --- & {\bf 8} & 1 & {\bf 7} & 1824 \\
\hline
{\bf s400} (183 / 186) & {\bf $\geq$ 3} & --- & --- & {\bf 6} & 0 & {\bf 5} & 273 \\
\hline
{\bf s420} (212 / 231) & {\bf $\geq$ 3} & --- & --- & {\bf 9} & 0 & {\bf 8} & 454 \\
\hline
{\bf s444} (202 / 205) & {\bf $\geq$ 3} & --- & --- & {\bf 6} & 0 & {\bf 5} & 385 \\
\hline
{\bf s510} (217 / 236) & {\bf $\geq$ 3} & --- & --- & {\bf 23} & 1 & {\bf 20} & 2082 \\
\hline
{\bf s526} (214 / 217) & {\bf $\geq$ 3} & --- & --- & {\bf 8} & 1 & {\bf 7} & 1715 \\
\hline
{\bf s641} (398 / 433) & --- & --- & --- & {\bf 7} & 1 & {\bf 7} & 1611 \\
\hline
{\bf s713} (412 / 447) & --- & --- & --- & {\bf 7} & 1 & {\bf 7} & 1800 \\
\hline
{\bf s820} (294 / 312) & {\bf $\geq$ 3} & --- & --- & {\bf 13} & 3 & {\bf 12} & 2846 \\
\hline
{\bf s832} (292 / 310) & {\bf $\geq$ 3} & --- & --- & {\bf 12} & 3 & {\bf 11} & 2575 \\
\hline
{\bf s838} (422 / 457) & {\bf $\geq$ 3} & --- & --- & {\bf 16} & 1 & {\bf 15} & 2046 \\
\hline

\end{tabular}
%\end{center}
%\caption{ISCAS 89 benchmarks}
%\label{tab:iscas89}
%\end{sidewaystable}
%\end{table}

\setlength\extrarulesep{0pt}


==> graphics/tw_hw.tex <==

\begin{figure}[t]
\begin{center}
 
\input{graphics/tw_hw.pstex_t}

\caption{Tree and hypertree decompositions}
\label{fig:tw_hw}
\end{center}
\end{figure}


